Dynamic Forecasting of Conversation Derailment

Online conversations can sometimes take a turn for the worse, either due to systematic cultural differences, accidental misunderstandings, or mere malice. Automatically forecasting derailment in public online conversations provides an opportunity to take early action to moderate it. Previous work in this space is limited, and we extend it in several ways. We apply a pretrained language encoder to the task, which outperforms earlier approaches. We further experiment with shifting the training paradigm for the task from a static to a dynamic one to increase the forecast horizon. This approach shows mixed results: in a high-quality data setting, a longer average forecast horizon can be achieved at the cost of a small drop in F1; in a low-quality data setting, however, dynamic training propagates the noise and is highly detrimental to performance.

==> data.tex <==
\paragraph{Wikipedia Abusive Conversations (WAC)}

In the task of abuse detection a prediction is made as to whether a personal attack (among other things) is present in an \textit{observed} comment. This is often done over comments in isolation, which makes most data sets for the task unusable for forecasting derailment, where we need to make a prediction for a personal attack \textit{before it has been observed}. \citet{wac} recently introduced the Wikipedia Abusive Content (WAC) data set which targets abuse detection \textit{in context} and contains 51,760 conversations with at least one comment annotated for a personal attack. The resource is build from comments extracted from Wikipedia Talk Pages and annotated in isolation, whose context has then been recovered with reference to the WikiConv corpus of raw Wikipedia Talk Page conversations. The availability of context in WAC allows us to adapt this resource to the task The , however,  which makes it suitable for forecasting derailment as well, albeit with some extensive filtering. 

%WAC contains 51,760 conversations with at least one comment annotated for a personal attack, with 13.2\% of annotated comments having a positive label. 

\subsection{Conversations Gone Bothersome (\cgb)}

In this subsection we describe the process of building \cgb, a dataset for forecasting derailment derived from the WAC dataset for abuse detection. In this process we replicate some properties of \cga and \cmv but also make some design choices different from  \citet{awry} and \citet{trouble}. The WAC corpus contains Wikipedia Talk Page conversations in their raw form with various metadata about edits made to the comments---these are preprocessed as described in Appendix~\ref{app:data} to obtain coherent conversations.
% Regarding the requirement that the attack \textit{comes from within}, we see the value in this, especially considering the large number of trolls on Wikipedia, who randomly insert themselves in conversations in unpredictable patterns. We ease the requirement here as well though, to permit any conversation where the abusive comment comes from a user who has previously participated in the conversation (but not necessarily in the initial exchange). With these considerations in mind, we process the WAC dataset as described below.   

\paragraph{Noise}

Since only a few comments in a conversation are annotated, there is a risk of some unnanotated comments containing a personal attack---a problem that holds for the \cmv~ data set. %If such comments occur prior to the first positively labelled comment in a conversation, this would lead to a wrong perception of when the derailment began. If such comments occur anywhere in a conversation with only negative labels, it would make the conversation a false negative.
To address this, we refer to the Perspective API toxicity scores already available in WAC. We interpret any score below 0.4 to mean that no toxicity was detected, and filter out any conversations that contain scores above that threshold for unannotated comments. This procedure provides to guarantee that all unannotated personal attacks will be filtered out, as a personal attack need not necessarily be toxic. We do, however, find that X percent of personal attacks in \cga~ have a toxicity score over 0.4.  The procedure also likely removes some instances where toxicity occurs without being a personal attack---but we find that only Y percent of comments with toxicity score over 0.4 in \cga~ are not labeled as personal attacks. We can therefore conclude that the procedure is sufficiently robust to license its usage.

\paragraph{Conversation length} 

We believe that it is permissible to lax the requirement of previous data sets that a `civil' beginning should consist of two turns---as long as the conversation opens with a civil comment, we are in a position to make a forecast for a potential derailment. And there is no reason to disregard attacks that happen on the second turn of a conversation. This allows the minimum conversation length to be two instead of three turns and we discard only single-turn conversations from WAC. 

With this criterion in place, filtering out troll attacks is more challenging, however: in \cga~ and \cmv~ that was accomplished by ensuring that the attack came from within the conversation, but in two-turn conversations the second comment will always come from a `new' user. We manually check all two-turn conversations and discard ten troll attacks: these constitute comments where the same insulting word, phrase or sentence is repeated multiple times, often written in all caps, with no clear reference to the first comment in the conversation. 

\paragraph{Balancing and controls}

For every conversation with a positive label, we find a negative counterpart aiming to match both the topic and the length of the conversation if possible. Length control was not implemented in either \cga~ or \cmv, but we consider that an important factor as well, since that could be another source of bias. Where exact matching of topic and length is not possible, we prioritise the topic and if all else fails, we only match the length of the conversations. 
The 2,370 pairs of conversations that emerge from the steps described above are split 60-20-20 for training, validation and testing, with test pairs being drawn from the subset of pairs perfectly matched for both topic and length. 



\paragraph{Final notes}
It is worth noting that due to the combined approach of manual annotation of comments in isolation and subsequent automatic filtering of conversations, \cgb~ can be considered of lower quality than \cga, which is fully annotated, and of higher quality than \cmv, which lacks any noise filtering.
